From Perfect to Noisy World Simulation: Customizable Embodied Multi-modal Perturbations for SLAM Robustness Benchmarking

Embodied agents require robust navigation systems to operate in unstructured environments, making the robustness of Simultaneous Localization and Mapping (SLAM) models critical to embodied agent autonomy. While real-world datasets are invaluable, simulation-based benchmarks offer a scalable approach for robustness evaluations. However, the creation of a challenging and controllable noisy world with diverse perturbations remains under-explored. To this end, we propose a novel, customizable pipeline for noisy data synthesis, aimed at assessing the resilience of multi-modal SLAM models against various perturbations. The pipeline comprises a comprehensive taxonomy of sensor and motion perturbations for embodied multi-modal (specifically RGB-D) sensing, categorized by their sources and propagation order, allowing for procedural composition. We also provide a toolbox for synthesizing these perturbations, enabling the transformation of clean environments into challenging noisy simulations. Utilizing the pipeline, we instantiate the large-scale Noisy-Replica benchmark, which includes diverse perturbation types, to evaluate the risk tolerance of existing advanced RGB-D SLAM models. Our extensive analysis uncovers the susceptibilities of both neural (NeRF and Gaussian Splatting -based) and non-neural SLAM models to disturbances, despite their demonstrated accuracy in standard benchmarks. Our code is publicly available at https://github.com/Xiaohao-Xu/SLAM-under-Perturbation.

==> figs/fig_depth_perturbation.tex <==
\begin{figure}[t!]
	\centering
\includegraphics[width=0.48\textwidth]{figures/depth-perturbation.pdf} 
	\caption{\textbf{Taxonomy of sensor-level perturbations for depth imaging}. We introduce four perturbations to mimic the perception noises (\textit{i.e.}, random noises and missing) and the limited perception field of depth sensors.
}
	\label{fig:depth-corruption}
\end{figure}

==> figs/fig_perturb_severity_compare.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/fig_severity_preliminary.png} 
	\caption{Comparison between perturbation severity (low, middle, high).\textcolor{blue}{ TODO: remake, 4+1 methods, static mode (no low mid high))}}%\vspace{-2mm}
	\label{fig:image-severity-coslam-compare}
\end{figure}

==> figs/fig_perturb_type_compare.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.44\textwidth]{figures/fig_perturb_type_preliminary.png} 
	\caption{Comparison between perturbation types.\textcolor{red}{ (remake-later)}}%\vspace{-2mm}
	\label{fig:image-type-coslam-compare}
\end{figure}

==> figs/fig_perturbation_taxonomy_for_SLAM.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/perturbation_taxonomy.pdf} 
	\caption{\textbf{Taxonomy of perturbations for SLAM.} Given (\textbf{a}) the original (clean) sensor stream and (\textbf{b}) trajectory, our noisy data synthesis pipeline enables the simulation of (\textbf{c}) sensor corruption (for both RGB images and depth maps), (\textbf{d}) trajectory perturbations, and (\textbf{e}) multi-sensor misalignment for the multi-modal input setting.\textcolor{red}{remake this figure to illustrate the relationship between different perturbations and their order in the synthesis procedure}}
	\label{fig:all-perturb-taxonomy}
\end{figure}

==> figs/fig_qualitative_result_trajectory_perturbation.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figures/traj-ptb-qualitative_all.pdf} 
	\caption{\textbf{Illustration of trajectory deviations under different severity levels, the faster motion effect, and the multi-sensor misalignment effect.} We also show qualitative results of an advanced real-time SLAM model, \textit{i.e.}, CO-SLAM~\cite{coslam}. The impact of translation deviation, rotation deviation, {faster motion}, and sensor misalignment perturbations is assessed. For clarity, we visualize the projected trajectory on the horizontal x-y plane derived from the 3D trajectory, which shows that slight trajectory deviations can have a  significant impact on the trajectory estimation performance, measured by ATE.}%\vspace{-2mm}
	\label{fig:taxonomy-trajectory-misalign-perturbation}
\end{figure*} 



==> figs/fig_result_fast_motion.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/qualitative_result_coslam_faster_motion.png} 
	\caption{Effect of \textit{Faster Motion} perturbation on the performance for each scene in the Replica Dataset. We visualize the 3D point cloud reconstruction of an environment, accompanied by graphs comparing predicted trajectory (in blue) with ground truth trajectory (in black).}%\vspace{-2mm}
	\label{fig:faster-motion-coslam-qualitative}
\end{figure}

==> figs/fig_teaser.tex <==
\begin{figure}[t]
	\centering	\includegraphics[width=0.48\textwidth]{figures/teaser-customizable-slam.pdf} 
	\caption{\textbf{Overview of customizable robustness evaluation pipeline SLAM for SLAM {u}nder {p}erturbation}. Using customized robot slam systems and noisy world configurations, which includes the proposed comprehensive perturbation toolbox for SLAM task, customized robustness benchmark can be derived via noisy data synthesis. Then, the robustness of the slam model can be evaluated, which provides guidance for the  robot system optimization and the  feasibility judgement  of SLAM deployment under certain \textit{noisy world}.\textcolor{red}{remove this figure}}
	\label{fig:teaser}
\end{figure}

==> figs/simulator_pipeline.tex <==
\begin{figure*}[t]
	\centering	\includegraphics[width=\textwidth]{figures/RobuSLAM_Simulation_Pipeline_0111.pdf} 
	\caption{\textbf{Overview of noisy data synthesis  pipeline for SLAM evaluation under perturbation.} Given the customizable robot system  and global trajectory, the local trajectory of each sensor can be generated via physical engine. Then, trajectory perturbation composer introduces deviations to mimic locomotion perturbations. Afterwards, the render combines sensor configurations, perturbed local trajectories, and 3D scene models to generate clean sensor streams. Finally, sensor perturbation composer introduces corruptions to the sensor streams, which derives perturbed data for SLAM robustness benchmark.}%\vspace{-2mm}
	\label{fig:overview-simulator-pipeline}
\end{figure*}

==> src/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  
    \answerYes{Please refer to the abstract section and the introduction section (see Section~\ref{sec:introduction}).}
  \item Did you describe the limitations of your work?
  
    \answerYes{See limitations and future work in Section~\ref{sec:conclusions}.}
  \item Did you discuss any potential negative societal impacts of your work?
  
    \answerYes{See Appendix Sec. G of Supp. Material.}% ~\ref{sec:social-impact}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...

    \answerNA{We are not including theoretical results.}

\item If you ran experiments (e.g., for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  
    \answerYes{We have provided detailed code and instructions via an open-source GitHub repository: \url{https://github.com/Xiaohao-Xu/SLAM-under-Perturbation}. Additionally, implementation details are included in the Experiment section (see Section~\ref{sec:experiment}) and the Appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  
    \answerYes{Please refer to the experiment section (see Section~\ref{sec:experiment}).}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
  
    \answerYes{See Appendix Sec. K of Supp. Material.}% ~\ref{sec:detailed-result-with-error-bar}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
  
    \answerYes{See Appendix Sec. C.4 of Supp. Material.}% ~\ref{subsec:hardware}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  
    \answerYes{Please refer to the experiment section (see Section~\ref{sec:experiment}).}
  \item Did you mention the license of the assets?
  
    \answerYes{Please refer to the Public Resources Used section of the Appendix (Appendix Sec. I of Supp. Material).}% ~\ref{sec:license}
  \item Did you include any new assets either in the supplemental material or as a URL?
  
    \answerYes{We proposed new assets (i.e., new benchmark and code) and mentioned the URL and GitHub repository in the Availability and Maintenance section of the Appendix (Appendix Sec. H of Supp. Material).}% ~\ref{sec:availablility-maintenance}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  
    \answerYes{The data we used are publicly available datasets for academic purposes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  
    \answerNA{The dataset we used does not contain such content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...

    \answerNA{We do not use crowdsourcing or conducted research with human subjects.}

\end{enumerate}

==> tables/table_make_figure.tex <==
\begin{table}[t]

    \centering
    \setlength{\tabcolsep}{2.5mm}
    \caption{Trajectory estimation error (ATE [m]) of monocular (\textbf{Top}) and RGBD (\textbf{Bottom}) SLAM under faster motion.}%\vspace{-3mm}
        \label{tab:faster-motion-perturbation}
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{l|c|ccc}
    \toprule \toprule
     {\textbf{Speed-up Ratio}}
     & {$\textbf{1}\times$} & \textbf{$\textbf{2}\times$} & \textbf{$\textbf{4}\times$} & \textbf{$\textbf{8}\times$}    \\ \midrule 
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{{0.0042}}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0048}}$ 
    \\
    \midrule %\midrule
    iMAP (RGBD)~\cite{imap}& $0.1209$ & $0.4675$ & $0.9445$ & $${1.0000}$$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam} & $0.0147$ & $0.1702$ & $${1.0000}$$ & $${1.0000}$$  
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.1062$ & $0.9510$ & $${1.0000}$$ 
    \\
    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0046}}$ & $\textbf{{0.0050}}$  
    \\
SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $0.0184$ & $${1.0000}$$ & $${1.0000}$$ 
    \\
    \bottomrule \bottomrule
  \multicolumn{5}{l}{{\textbf{1}) Notice that the sensor stream under faster motion effect is synthesized}}  \\
  \multicolumn{5}{l}{{ by downsampling the original sensor stream. Thus, the derived sensor stream}}\\
     \multicolumn{5}{l}{{ under faster motion is shorter than the original one.}} \\

    \end{tabular}% Models with the best performance are in \textbf{bold}
    
}\end{table}




\begin{table}[t]
\caption{Trajectory estimation error (ATE [m]) under {depth imaging perturbation} for RGBD SLAM methods. }
\label{tab:depth-perturb}
\centering 
\setlength{\tabcolsep}{0.6mm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c|cccc}
    \toprule \toprule   
    \multirow{2}{*}{\textbf{Method}} &    \multirow{2}{*}{\textbf{Clean}}
     &  {\textbf{Gaussian}}   & {\textbf{Edge}} & 
  {\textbf{Random}}  & {\textbf{Range}}      \\  
 & & \textbf{Noise} & \textbf{Erosion} & \textbf{Missing} & \textbf{Clipping}\\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $${1.0000}$$ & $0.0307$ & $0.1083$  & $0.2438$ 
    \\ 
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $${1.0000}$$ & $0.0149$ & $0.0154$  & $0.1183$ 
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.5794$ & $0.0096$ & $0.0094$  & $0.0122$ 
    \\
    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{0.0378}$ & $0.0046$ & ${0.0046}$ & $\textbf{{0.0045}}$   
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $${1.0000}$$ & $\textbf{{0.0042}}$ & $\textbf{0.0042}$  
  & ${0.0048}$ 
    \\
    \bottomrule \bottomrule
    \multicolumn{6}{l}{{$${1.0000}$$ indicates  completely unacceptable trajectory estimation performance,}} \\
        \multicolumn{6}{l}{{\textit{i.e.}, ATE $\geq$ 1.0 [m]. Models with the best performance are in \textbf{bold}}}
    \end{tabular}
}
 
\end{table}




\begin{table*}[th]
    \centering

       \caption{Trajectory estimation error (ATE [m]) under trajectory-level deviation.}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \toprule \toprule
     \textbf{Rotate [$\deg$]} & \multirow{2}{*}{\textbf{Clean}}  & \multicolumn{3}{c|}{\textbf{\textit{0}}} & \multicolumn{4}{c|}{\textbf{\textit{1}}} & \multicolumn{4}{c|}{\textbf{\textit{3}}} & \multicolumn{4}{c}{\textbf{\textit{5}}}
    \\ \cmidrule{1-1} \cmidrule{3-5} \cmidrule{6-9} \cmidrule{10-13} \cmidrule{14-17}
     \textbf{Translate  [$m$]} &  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}}  & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} & \textit{\textbf{0}} & \textit{\textbf{0.0125}} &\textit{\textbf{0.025}} & \textbf{\textit{0.05}} 
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0084}$ & $\textbf{0.0077}$ & $\textbf{0.0091}$ & $\textbf{0.0083}$ & $\textbf{0.0079}$ & $\textbf{0.0082}$ & $\textbf{0.0094}$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$  
    \\ \midrule
   iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.0334$ & $0.1386$ & $0.0442$ & $0.2438$ & $0.2135$ & $0.3754$ & $0.2801$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$   \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.5812$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ 
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$ & $0.0420$ & $0.0848$ & $0.3087$ & $0.4579$ & $0.5069$ & $0.2998$ & $0.5040$ & $0.6443$ & $0.6630$ & $0.7532$ & $0.5772$ & $0.8457$ & $0.7966$ & $0.8277$ & $${1.0000}$$ 
    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & ${0.0046}$ & $\textbf{0.0082}$ & $\textbf{0.0082}$ & $\textbf{0.0081}$ & $\textbf{0.0080}$ & $\textbf{0.0080}$ & $\textbf{0.0078}$ & $\textbf{0.0077}$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$  
    \\
SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $0.0545$ & $0.0980$ & $0.2964$ & $0.297F$ & $0.2272$ & $0.2313$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ & $${1.0000}$$ % \\
    \\ 

    \bottomrule \bottomrule

          \multicolumn{17}{l}{{Notation  represents settings that include failure sequences where no final trajectory is generated due to tracking loss. The number in front of  represents the}}\\
     \multicolumn{17}{l}{{ average ATE as failure sequences are set as a value of 1.0. Notation $${1.0000}$$ indicates completely unacceptable trajectory estimation performance, \textit{i.e.}, ATE $\geq$ 1.0 [m].  }}\\ 
    \end{tabular}
}
         \label{tab:trajectory-perturbation_sr_metric}
\end{table*}% 








\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under static mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ 
       % \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$  & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$   & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\  \midrule
     \midrule

        GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$  & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & $0.045$ & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\   
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}






\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under static mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ 
       % \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
    iMAP (RGBD)~\cite{imap} & $0.1209$  & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$   & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\ 
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Trajectory estimation error (ATE [m]) under Dynamic mode of image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc|cccc|cccc|cccc}
    \toprule \toprule
   Mean &  Clean  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contrast} & \textbf{JPEG}  & \textbf{Pixelate}
    \\\midrule\midrule

        GO-SLAM (Mono)~\cite{zhang2023goslam} & $\textbf{0.0039}$  & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    iMAP (RGBD)~\cite{imap} & $0.1209$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM (RGBD)~\cite{niceslam}& $0.0147$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM (RGBD)~\cite{coslam}& $0.0090$  & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM (RGBD)~\cite{zhang2023goslam} & $0.0046$  & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S (RGBD)~\cite{keetha2023splatam}& $\textbf{0.0045}$  & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & $0.045$ & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\   
    \bottomrule  \bottomrule

    \end{tabular}
}
\end{table*}










==> tables/table_sensor_perturb_performance_all.tex <==

\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office0)}

\label{tab:sensor_perturb_benchmark}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office1)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office2)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office3)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}

\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (office4)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room0)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}





\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room1)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Per-scene Sensor-level perturbation benchmarking (ATE) on Replica (room2)}

\label{tab:sensor_recon}
\centering\setlength{\tabcolsep}{1.0mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|cccc|cccc|cccc}
    \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Mean}} & \multicolumn{5}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Weather Effect}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{3-7} \cmidrule{8-11} \cmidrule{12-15} \cmidrule{16-19}
    &  & \textbf{Zoom} & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{18}{c}{Monocular Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\ \midrule
        \multicolumn{18}{c}{RGBD Setting}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    CO-SLAM~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    GO-SLAM~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam~\cite{orbslam3}& $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    \bottomrule
    \end{tabular}
}
\end{table*}




